Farthest points on flat surfaces

We consider the distance function from an arbitrary point $p$ on a flat surface, and determine the set $F_{p}$ of all \emph{farthest points} (i.e., points at maximal distance) from $p$.

==> Macros.tex <==
% V 2.1
\newcommand{\nc}{\newcommand}
\newcommand{\df}{\def}
\RequirePackage{ifthen}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%racourciss divers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\df\ie#1{{\mbox{{\it i.\hspace{0.06em}e.}\ifthenelse{\equal{#1}{,}}{\hspace{0.06em},}{\ #1}}}}
\df\eg#1{{\mbox{{\it e.\hspace{0.06em}g.}\ifthenelse{\equal{#1}{,}}{\hspace{0.06em},}{\ #1}}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Citations dans Theorem
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\cit}[2][]{\ifthenelse{\equal{#1}{}}{{\rm \cite{#2}}}{{\rm \cite[#1]{#2}}}}

\makeatletter

%%%%%%%%%TURNED-M

\newcommand{\most@textstyle}{\hspace{.07em plus .01 em minus .01em}\rule[-.1pt]{.35pt}{1.63ex}\hspace{-.315 em}\wedge\hspace{-.315 em}\rule[-.1pt]{.35pt}{1.63ex}\hspace{.15em plus .05em minus .05em}}

\newcommand{\most@scriptstyle}{\hspace{.05705em plus .00815 em minus .00815em}\rule[-.1pt]{.33pt}{1.139ex}\hspace{-.07 em}\wedge\hspace{-.07 em}\rule[-.1pt]{.33pt}{1.139ex}\hspace{.12225em plus .04075em minus .04075em}}

\newcommand{\most@scriptscriptstyle}{\hspace{.05075em plus .00725 em minus .00725em}\rule[-.1pt]{.32pt}{0.815ex}\hspace{-.063 em}\wedge\hspace{-.065 em}\rule[-.1pt]{.32pt}{0.815ex}\hspace{.10875em plus .03625em minus .03625em}}

\newcommand{\most}{\mathchoice{\most@textstyle}{\most@textstyle}{\most@scriptstyle}{\most@scriptscriptstyle}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Gestions des {|}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% usage:  \set(: xyz\in XYZ | xyz is something :) 
%
%Note: \set[xx](: ...| ...:) is for backward compatibility, xx is ignored.
%Note: \seti is an alias of \set, still for backward compatibility
%Note: If set are nested, inner sets must be enclosed in braces: {\set(:...|...:)}


\newlength{\Set@LH}
\newlength{\Set@RH}
\newlength{\Set@LD}
\newlength{\Set@RD}
\newlength{\Set@NoPar@W}

\newsavebox{\Set@Box@R}
\newsavebox{\Set@Box@L}

\newcommand{\Set@@}[3]{%#3=math style
\sbox{\Set@Box@L}{\ensuremath{#3#1}}
\sbox{\Set@Box@R}{\ensuremath{#3#2}}
\settoheight{\Set@LH}{\usebox{\Set@Box@L}}
\settodepth {\Set@LD}{\usebox{\Set@Box@L}}
\settoheight{\Set@RH}{\usebox{\Set@Box@R}}
\settodepth {\Set@RD}{\usebox{\Set@Box@R}}
\addtolength{\Set@LH}{\Set@LD}
\addtolength{\Set@RH}{\Set@RD}
{\def\mt{\rule[-\Set@LD]{0pt}{\Set@LH}\rule[-\Set@RD]{0pt}{\Set@RH}}
\settowidth{\Set@NoPar@W}{\ensuremath{#3\left.\mt\right.}}
\left\{\usebox{\Set@Box@L}\mt\right.\hspace{-.3\Set@NoPar@W}\left\vert\usebox{\Set@Box@R}\mt\right\}}
}


\def\Set@Smile(:#1|#2:){\mathchoice
{\Set@@{#1}{#2}{\displaystyle}}
{\Set@@{#1}{#2}{\textstyle}}
{\Set@@{#1}{#2}{\scriptstyle}}
{\Set@@{#1}{#2}{\scriptscriptstyle}}
}

\newcommand{\set}[1][]{\Set@Smile}
\newcommand{\seti}{\set}




\makeatother


